Linear Logic, the $\pi$-calculus, and their Metatheory: A Recipe for Proofs as Processes

Initiated by Abramsky [1994], the Proofs as Processes agenda is to establish a solid foundation for the study of concurrent languages, by researching the connection between linear logic and the $\pi$-calculus. To date, Proofs as Processes is still a partial success. Caires and Pfenning [2010] showed that linear propositions correspond to session types, which prescribe the observable behaviour of processes. Further, Carbone et al. [2018] demonstrated that adopting devices from hypersequents [Avron 1991] shapes proofs such that they correspond to the expected syntactic structure of processes in the $\pi$-calculus. What remains is reconstructing the expected metatheory of session types and the $\pi$-calculus. In particular, the hallmark of session types, session fidelity, still has to be reconstructed: a correspondence between the observable behaviours of processes and their session types, in terms of labelled transitions. In this article, we present $\pi$LL, a new process calculus rooted in linear logic. The key novelty of $\pi$LL is that it comes with a carefully formulated design recipe, based on a dialgebraic view of labelled transition systems. Thanks to our recipe, $\pi$LL offers the expected transition systems of session types, which we use to establish session fidelity. We use $\pi$LL to carry out the first thorough investigation of the metatheoretical properties enforced by linear logic on the observable behaviour of processes, uncovering connections with similarity and bisimilarity. We also prove that $\pi$LL and our recipe form a robust basis for the further exploration of Proofs as Processes, by considering different features: polymorphism, process mobility, and recursion.

==> preamble.tex <==
\makeatletter

\newcommand*{\installoption}[2][acmart]{
	\expandafter\newif\csname if#2\endcsname
	\@ifclasswith{#1}{#2}{
		\csname#2true\endcsname
	}{}
}
\newcommand*{\obeyoption}[2]{
	\csname if#2\endcsname\else\csname #1false\endcsname\fi
}
\newcommand*{\excludeoption}[2]{
	\csname if#2\endcsname\csname #1false\endcsname\fi
}
\makeatother

\installoption{highlight}
\installoption{appendix}
\installoption{final}
\installoption{draft}
\installoption{showframe}
\obeyoption{showframe}{draft}


\usepackage{aliascnt}
\usepackage{xparse}
\usepackage{etoolbox}
\usepackage{environ}
\usepackage{graphicx}

\def\deprecated#1{\PackageWarning{preamble}{Don't use ``#1''}{}}

\makeatletter
\newcommand{\IfLabelExistsTF}[3]{\@ifundefined{r@#1}{#3}{#2}}
\newcommand{\IfLabelExistsT}[2]{\IfLabelExistsTF{#1}{#2}{}}
\newcommand{\IfLabelExistsF}[2]{\IfLabelExistsTF{#1}{}{#2}}
\newcommand{\IfDefTF}[3]{\@ifundefined{#1}{#3}{#2}}
\newcommand{\IfDefT}[2]{\IfDefTF{#1}{#2}{}}
\newcommand{\IfDefF}[2]{\IfDefTF{#1}{}{#2}}
\makeatother



\def\proofltsskipamount{5pt}
\def\termltsskipamount{1\smallskipamount}
\def\envltsskipamount{1\smallskipamount}
\def\typerulesskipamount{.5\bigskipamount}
\providecommand\rulescalebox[2][]{#2} %

\usepackage{subfiles}
\usepackage{xr}
\usepackage{currfile}

\ifdefined\docroot\else
	\let\docroot\currfilepath
\fi

\newcommand\IfDocRootTF[2]{%
	\ifcurrfilepath{\docroot}{#1}{#2}%
}
\newcommand\IfDocRootT[1]{\IfDocRootTF{#1}{}}
\newcommand\IfDocRootF[1]{\IfDocRootTF{}{#1}}

\usepackage[utf8]{inputenc}
\usepackage{microtype}
\usepackage[normalem]{ulem}

\ifshowframe
\AtEndPreamble{%
	\usepackage{showframe}%
	\renewcommand*\ShowFrameColor{\color{black!50}}
	\renewcommand*\ShowFrameLinethickness{.5pt}
}
\fi

\usepackage{xcolor}

\colorlet{type}{blue!60!black}
\colorlet{process}{red!60!black}
\definecolor{light-gray}{gray}{0.8}

\colorlet{textcolor}{.}
\newcommand\usecolor[2]{\begingroup%
	\colorlet{uc@saved}{.}
	\color{#1}#2\color{uc@saved}
\endgroup}
\newcommand\cboxed[2]{\begingroup%
  \colorlet{cb@saved}{.}%
  \color{#1}%
  \boxed{\color{cb@saved}#2}%
\endgroup}

\usepackage{tikz}
\usepackage{hf-tikz} %
\usetikzlibrary{calc}

\usepackage[british]{babel}
\usepackage[all]{foreign}
\renewcommand\foreignabbrfont{}
\renewcommand\foreignfullfont{}
\defnotforeign[wrt]{{wrt}}
\defnotforeign[wl]{{wlog}}


\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{centernot}
\usepackage{scalerel}


\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\newcommand{\specialcell}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\ignorespaces\fi}
\makeatother

\allowdisplaybreaks

\makeatletter
\@ifundefined{minaw@}{\newdimen\minaw@}{}
\def\rightarrowtrianglefill@#1{\m@th\setboxz@h{$#1\relbar$}\ht\z@\z@
  $#1\copy\z@\mkern-6mu\cleaders
  \hbox{$#1\mkern-2mu\box\z@\mkern-2mu$}\hfill
  \mkern-6mu\mathord{\smash\rightarrowtriangle\vphantom{\rightarrow}}$}
\newcommand{\xrightarrowtriangle}[2][]{%
  \mathrel{\mathop{%
    \setbox\z@\vbox{\m@th
      \hbox{$\scriptstyle\;{#1}\;\;\,$}%
      \hbox{$\m@th\scriptstyle\;{#2}\;\;\,$}%
    }%
    \hbox to\ifdim\wd\z@>\minaw@\wd\z@\else\minaw@\fi{%
      \rightarrowtrianglefill@\displaystyle}}%
  \limits^{#2}\@ifnotempty{#1}{_{#1}}}%
}
\renewcommand{\xRightarrow}[2][]{\ext@arrow 0359\Rightarrowfill@{#1}{#2}}
\makeatother


\def\lclens{{[\llap(}}
\def\rclens{{\rlap)]}}


\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother



\usepackage{array}
\usepackage{xtab}
\xentrystretch{-0.2}
\usepackage{booktabs}
\usepackage{multicol}

\makeatletter
\def\crulefill#1{\leavevmode\leaders\hrule\@height#1 height 0.7ex depth \dimexpr0.4pt-0.7ex\hfill\kern0pt}
\makeatother


\def\headertext#1{
	\vspace{2pt}
	\crulefill{\lightrulewidth}\ \textsf{\small \emph{#1}}\ \crulefill{\lightrulewidth}
  \\[-2.7ex]%
}

\def\header{
 	\vspace{-1.6\smallskipamount}%
 	\rule[1\abovedisplayskip]{\textwidth}{\heavyrulewidth}%
}

\newcommand*{\footer}[1][1.6\belowdisplayskip]{%
	\rule[#1]{\textwidth}{\lightrulewidth}%
	\vspace{-1.6\smallskipamount}%
}

\usepackage{float}
\usepackage{placeins}
\usepackage{wrapfig}

\usepackage[inline]{enumitem}

\usepackage{nameref}

\usepackage[capitalise,nameinlink,noabbrev]{cleveref}
\makeatletter
\newcommand{\customlabel}[4][0]{%
	\protected@write\@auxout{}{\string\newlabel{#3}{{#4}{\thepage}{#4}{#3}{}}}%
	\protected@write\@auxout{}{\string\newlabel{#3@cref}{{[#2][#1][#1]#4}{\thepage}}}%
}
\newcommand{\phantomlabel}[4][0]{%
	\customlabel[#1]{#2}{#3}{#4}%
	\hypertarget{#3}{}%
}
\newcommand{\labelalias}[4][0]{
	\customlabel[#1]{#2}{#3}{#4}%
}
\newcommand{\crefv}[1]{%
	\begingroup\@cref@compressfalse\@cref@sortfalse\cref{#1}\endgroup%
}
\newcommand{\Crefv}[1]{%
	\begingroup\@cref@compressfalse\@cref@sortfalse\Cref{#1}\endgroup%
}
\newcommand{\crefabbrev}[1]{%
	\begingroup\@cref@abbrevtrue\cref{#1}\endgroup%
}
\makeatother

\AtEndPreamble{\hypersetup{
	final,
}}


\usepackage{proof-dashed}

\newcounter{rule}

\newcommand{\rname}[1]{\ensuremath{\textsc{\MakeLowercase{#1}}}}
\newcommand{\rlabel}[2]{{%
	\refstepcounter{rule}
	\customlabel[\therule]{infrule}{#2}{#1}%
	\hypertarget{#2}{#1}}}
\crefname{infrule}{rule}{rules}
\Crefname{infrule}{Rule}{Rules}

\newcommand{\rrelabel}[2]{\rlabel{\ref*{#1}}{#2}}
\newcommand{\rlabelfwd}[2]{
	\refstepcounter{rule}
	\customlabel[\therule]{infrule}{#2}{\ref{#1}}%
}


\AtEndPreamble{
	\theoremstyle{acmplain}
  \newtheorem{exercise}[theorem]{Exercise}
	\newtheorem{fact}[theorem]{Fact}
	\theoremstyle{acmdefinition}
	\newtheorem{remark}[theorem]{Remark}
}

\crefname{proof}{proof of}{proofs of}
\Crefname{proof}{Proof of}{Proofs of}

\newcommand{\prooflabel}[2]{{%
	\customlabel{proof}{#2}{\cref*{#1}}%
	\hypertarget{#2}{}}}

\makeatletter
\newcounter{proofatend@statemet}

\patchcmd{\@addmarginpar}{\ifodd\c@page}{\ifodd\c@page\@tempcnta\m@ne}{}{}
\reversemarginpar

\newcommand*\fixstatement[2][Proof of]{%
	\expandafter\preto\csname end#2\endcsname{%
		\global\def\proofatend@proofof{#1}%
		\stepcounter{proofatend@statemet}%
		\label{proofatend:\theproofatend@statemet}%
		\if\proofatend@mode\proofatend@postpone%
		\IfLabelExistsTF{proofatend:proof-\theproofatend@statemet}{%
			\marginpar{\hyperref%
				[proofatend:proof-\theproofatend@statemet]%
				{\rotatebox[origin=c]{-90}{$\triangle$}}
			}%
		}{}%
		\fi%
}}

\def\proofatend@toks{1000}
\newcounter{proofatend@stored}
\newcounter{proofatend@printed}

\let\proofatend@omit0
\let\proofatend@inplace1
\let\proofatend@postpone2

\newcommand{\omitproofs}{\global\let\proofatend@mode\proofatend@omit}
\newcommand{\postponeproofs}{\global\let\proofatend@mode\proofatend@postpone}
\newcommand{\keepproofs}{\global\let\proofatend@mode\proofatend@inplace}

\ifappendix
\postponeproofs
\else
\omitproofs
\fi

\NewEnviron{proofatend}[1][Proof]{\ignorespaces%
	\if\proofatend@mode\proofatend@inplace%
		\begin{proof}[#1]\BODY\end{proof}%
	\else\if\proofatend@mode\proofatend@postpone%
		\edef\next{%
			\noexpand\begin{proof}[{\proofatend@proofof~\noexpand\cref{proofatend:\theproofatend@statemet}}]%
			\noexpand\phantomsection%
			\noexpand\label{proofatend:proof-\theproofatend@statemet}%
			\unexpanded\expandafter{\BODY}}%
		\global\toks\numexpr\proofatend@toks+\value{proofatend@stored}\relax=\expandafter{\next\end{proof}}%
		\stepcounter{proofatend@stored}%
	\fi\fi\ignorespacesafterend}

\NewDocumentCommand{\omittedproofs}{o}{%
	\ifnum\value{proofatend@printed}<\value{proofatend@stored}%
		\IfNoValueF{#1}{#1}%
		\count@=\value{proofatend@printed}%
		\loop%
			\the\toks\numexpr\proofatend@toks+\count@\relax%
			\stepcounter{proofatend@printed}%
			\ifnum\count@<\value{proofatend@stored}%
				\advance\count@\@ne%
		\repeat%
	\fi%
}
\makeatother

\AtEndPreamble{
	\fixstatement{theorem}
	\fixstatement{proposition}
	\fixstatement{corollary}
	\fixstatement{lemma}
	\fixstatement{fact}
  \fixstatement[Solution to]{exercise}
}

\bibliographystyle{ACM-Reference-Format}
\citestyle{acmauthoryear}

\usepackage[
	obeyFinal,   %
	textsize=tiny,
	colorinlistoftodos,
	prependcaption
]{todonotes}
\newcommand{\unsure}[2][]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommand{\change}[2][]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommand{\info}[2][]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan,#1]{#2}}
\newcommand{\improvement}[2][]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}


\makeatletter
\def\new@acronym#1#2{%
  \expandafter\def\csname#1@acr\endcsname{\text{\upshape #2}\xspace}%
  \expandafter\def\csname#1\endcsname{{\upshape #2}\xspace}}
\def\new@acronymexp#1#2{\expandafter\def\csname#1@exp\endcsname{{#2}}}
\NewDocumentCommand{\newacronym}{o m o}{%
	\IfNoValueTF{#1}{\def\n{#2}}{\def\n{#1}}
  \new@acronym{\n}{#2}
  \IfNoValueF{#3}{\new@acronymexp{\n}{#3}}
}
\def\acronym#1{\csname#1@acr\endcsname}
\def\expandacronym#1{\csname#1@exp\endcsname}
\makeatother

\newacronym{CP}[Classical Processes]
\newacronym{MCP}[Multiplicative Classical Processes]
\newacronym[CPZero]{CP\textsubscript{0}}[Non-Polymorphic Classical Processes]
\newacronym{CHOP}[Classical Higher-Order Processes]
\newacronym{HCP}[Hypersequent Classical Processes]
\newacronym{DHCP}[Hypersequent Classical Processes with Delayed Actions]
\newacronym[HOpi]{HO$\pi$}[Higher-Order $\pi$-calculus]
\newacronym{CLL}[Classical Linear Logic]
\newacronym{MCLL}[Multiplicative Classical Linear Logic]
\newacronym[CLLZero]{CLL\textsubscript{0}}[Quantifier-free Classical Linear Logic]
\newacronym[CLLZeroOne]{CLL\textsubscript{01}}[Classical Linear Logic with first-order quantifiers]
\newacronym{ILL}[Intuitionistic Linear Logic]
\newacronym[lts]{lts}[labelled transition system]
\newacronym[pill]{$\pi$LL\xspace}
\newacronym[hopill]{HO$\pi$LL\xspace}[Higher-Order \pill]
\newacronym[polypill]{Poly$\pi$LL\xspace}[Polymorphic \pill]
\newacronym[pimll]{$\pi$MLL\xspace}[Multiplicative \pill]
\newacronym[pimell]{$\pi$MELL\xspace}
\newacronym[pimall]{$\pi$MALL\xspace}


\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\img}{img}

\DeclareMathOperator{\prfhyp}{hyp}
\DeclareMathOperator{\prfproc}{proc}
\DeclareMathOperator{\cn}{cn} %
\DeclareMathOperator{\fn}{fn} %
\DeclareMathOperator{\bn}{bn} %
\DeclareMathOperator{\pv}{pv} %
\DeclareMathOperator{\fv}{fv} %
\DeclareMathOperator{\fpv}{fpv} %
\DeclareMathOperator{\ftv}{ftv} %
\DeclareMathOperator{\ppnf}{parnf} %

\makeatletter
\DeclareMathOperator{\bigtensor}{{\textstyle\bigotimes}}
\DeclareMathOperator{\bigparr}{\scalerel*{\parr}{\bigtensor}}
\makeatother

\makeatletter
\newcommand{\enc}{\@ifstar{\enc@}{\enc@@}}
\def\enc@#1{\left\llbracket \mkern-7mu\array{c}#1\endarray\mkern-7mu \right\rrbracket}
\def\enc@@#1{\llbracket#1\rrbracket}
\makeatother

\DeclareMathOperator{\disenop}{dis}  %
\DeclareMathOperator{\packop}{pack}  %
\DeclareMathOperator{\unpackop}{unpack}

\newcommand{\disen}[1]{\disenop(#1)}
\newcommand{\pack}[3][]{\packop^{#1}_{#2}(#3)}
\newcommand{\unpack}[3][]{\unpackop^{#1}_{#2}(#3)}


\def\crel#1{\mathrel{\mathcal{#1}}}


\def\disjoint{\mathrel{\#}}

\let\defeq\triangleq
\edef\defiff{\stackrel{\triangle}{\iff}}

\edef\aleq{\mathbin{=_{\alpha}}}
\let\congr\equiv
\def\tyeq{\mathrel{\dashv\vdash}}
\let\bis\approx
\let\sbis\sim
\let\bcong\approxeq
\let\deneq\bumpeq
\def\ssimby{\lesssim}
\def\ssims{\gtrsim}
\def\simby{\lessapprox}
\def\sims{\gtrapprox}

\let\reducesto\rightarrow
\def\breducesto{\mathbin{{\rightarrow}_\beta}}
\def\kreducesto{\mathbin{{\rightarrow}_\kappa}}

\makeatletter
\def\lto#1{\xrightarrow{\lbox{#1}}} %
\def\slto#1{\xRightarrow{\lbox{#1}}} %
\def\notlto#1{\centernot{\xrightarrow{\lbox{#1}}}}
\def\notslto#1{\centernot{\xRightarrow{\lbox{#1}}}}
\newcommand\lbox[2][.8em]{
	\sbox0{$\scriptstyle #2$}
	\ifdim \wd0 < #1%
		\mathmakebox[#1]{\usebox0}%
	\else%
		\mathmakebox[\wd0]{\usebox0}%
	\fi%
}

\newcommand{\plto}{%
	\@ifstar{\plto@v\downarrow}{\plto@h\lto}%
}
\newcommand{\pslto}{%
	\@ifstar{\plto@v\Downarrow}{\plto@h\slto}%
}
\def\pboxcolor{black!10}
\def\pbox#1{\cboxed{\pboxcolor}{\mspace{-10mu}\array{c}#1\endarray\mspace{-10mu}}}
\let\plto@b\pbox
\def\plto@h#1#2#3#4{%
	\plto@b{#2}%
	#1{#3}%
	\plto@b{#4}%
}
\def\plto@v#1#2#3#4{%
	\array[b]{l}%
		\plto@b{#2}%
		\\%
		\quad%
		\cboxed{white}{\scriptstyle\left#1\cboxed{white}{\scriptstyle#3}\right.}\\%
		\plto@b{#4}%
	\endarray%
}
\newcommand{\notplto}[2]{%
	\plto@b{#1} \notlto{#2}%
}
\def\pvlto#1{\quad\cboxed{white}{\scriptstyle\left\plto@v\downarrow\cboxed{white}{\scriptstyle#1}\right.}}%
\def\pvlto#1{\quad\cboxed{white}{\scriptstyle\left\plto@v\Downarrow\cboxed{white}{\scriptstyle#1}\right.}}%
\makeatother

\newenvironment{drules}
  {\highlight\spreadlines{\proofltsskipamount}\small\csname gather*\endcsname}
  {\csname endgather*\endcsname\endspreadlines\endhighlight}

\crefname{ltstrace}{trace}{traces}
\Crefname{ltstrace}{Trace}{Traces}
\crefalias{equation}{ltstrace}


\def\terminates{{\downharpoonright}}
\def\diverges{{\upharpoonright}}
\def\mayterminate{{\Downharpoonright}}
\def\maydiverge{{\Upharpoonright}}


\def\phl#1{#1}%
\def\thl#1{#1}%
\def\nohl#1{#1}%
\newcommand{\hl}[1]{\highlight#1\endhighlight}
\ifhighlight
\newenvironment{highlight}
	{\ignorespaces%
	 \def\phl##1{\usecolor{process}{##1}}%
	 \def\thl##1{\usecolor{type}{##1}}%
	 \def\nohl##1{\usecolor{textcolor}{##1}}}%
	{\def\phl##1{##1}%
   \def\thl##1{##1}%
   \def\nohl##1{##1}%
	 \ignorespacesafterend}
\else
\newenvironment{highlight}{\ignorespaces}{\ignorespacesafterend}
\fi

\newenvironment{bnftable}[3][\phl]
	{\begin{bnftable2}[#1]{#2}{#3}{}}
	{\end{bnftable2}}

\newenvironment{bnftable2}[4][\phl]
	{\vskip\abovedisplayskip\rmfamily\flushleft\highlight%
	  \sbox0{$#2$}%
	  \sbox1{$#3$}%
 	  \sbox2{#4}%
	  \begin{xtabular*}{\textwidth}{%
	      >{\raggedleft$}m{\wd0}<{$}%
	      >{\raggedright$#1\begingroup}m{\wd1}<{\endgroup$}%
	      >{\it}l<{}@{\extracolsep{\fill}}
	      >{\hfill\it}m{\wd2}<{}}}
	{\end{xtabular*}\endhighlight\endflushleft\vskip\belowdisplayskip}


\newcommand*{\bang}{\mathord{!}}
\newcommand*{\query}{\mathord{?}}
\newcommand*{\tensor}{\otimes}
\newcommand*{\parr}{\mathbin{\bindnasrepma}}
\newcommand*{\with}{\mathbin{\binampersand}}
\newcommand*{\one}{1}
\newcommand*{\zero}{0}
\newcommand*{\dual}[1]{#1^{\bot}}
\newcommand{\provide}[1]{{[#1]}}
\newcommand{\assume}[1]{{\langle #1 \rangle}}

\newcommand*{\cht}[2]{\phl{#1}\nohl{\colon}\mspace{-2mu}\thl{#2}} %
\newcommand*{\pvt}[2]{\phl{#1}\nohl{\colon}\mspace{-2mu}\thl{#2}} %
\newcommand*{\emptyseq}{\bullet}
\newcommand*{\emptyhyp}{\varnothing}
\newcommand*{\emptyho}{\cdot}
\newcommand*{\hyp}[1]{\mathcal{#1}}

\let\seq\vdash
\newcommand*{\prf}[1]{\ensuremath{\mathcal{#1}}}
\def\ccolon{\mathrel{:\mspace{-1mu}:}}
\newcommand{\judge}[4][]{{}\nohl{\thl{#2} \seq_{\thl{#1}}} \phl{#3} \nohl{\ccolon} \thl{#4}}
\newcommand{\cpjudge}[2]{\judge[\text{\tiny\CP}]{}{#1}{#2}}


\newcommand*{\strip}[1]{\left\lfloor{#1}\right\rfloor}


\newcommand*{\minl}{\mathsf{i\mspace{-.7mu}n\mspace{-.7mu}l}}
\newcommand*{\minr}{\mathsf{i\mspace{-.7mu}n\mspace{-.7mu}r}}
\newcommand*{\asend}[2]{{#1[#2]}}
\newcommand*{\arecv}[2]{{#1(#2)}}
\newcommand*{\aclose}[1]{\asend{#1}{}}
\newcommand*{\await}[1] {\arecv{#1}{}}
\newcommand*\fixspace[2][2mu]{\mspace{#1}{#2}\mspace{#1}}
\newcommand*{\ainl}[1]{{#1}\fixspace{\triangleleft}{\minl}}
\newcommand*{\ainr}[1]{{#1}\fixspace{\triangleleft}{\minr}}
\newcommand*{\acoinl}[1]{{#1}\fixspace{\triangleright}{\minl}}
\newcommand*{\acoinr}[1]{{#1}\fixspace{\triangleright}{\minr}}
\newcommand*{\asendtype}[2]{\asend{#1}{#2}}
\newcommand*{\arecvtype}[2]{\arecv{#1}{#2}}
\newcommand*{\aclientuse}[2] {\query\asend{#1}{#2}}
\newcommand*{\aserveruse}[2] {\bang \arecv{#1}{#2}}
\newcommand*{\aclientdisp}[1]{\query\asend{#1}{}}
\newcommand*{\aserverdisp}[1]{\bang \arecv{#1}{}}
\newcommand*{\aclientdup}[3] {\query\asend{#1}{#2,#3}}
\newcommand*{\aserverdup}[3] {\bang \arecv{#1}{#2,#3}}
\newcommand*{\forwardop}{{\leftrightarrow}}
\newcommand*{\aforward}[3][]{{#2 \forwardop^{#1} #3}}
\newcommand*{\asendho}[2]{\asend{#1}{#2}}
\newcommand*{\arecvho}[2]{\arecv{#1}{#2}}
\newcommand{\asendfree}[2]{#1 \langle #2 \rangle}
\newcommand{\nil}{\boldsymbol{0}}
\let\forward\aforward
\newcommand*{\pp}{\mathbin{\boldsymbol{|}}}
\newcommand*{\resop}{\mathop{\boldsymbol{\nu}}}
\newcommand*{\res}[2]{{(\boldsymbol{\nu}{#1})\mspace{2mu}}{#2}}
\newcommand*{\prefixed}[2]{{#1.#2}}
\newcommand*{\send}[3]{\prefixed{\asend{#1}{#2}}{#3}}
\newcommand*{\recv}[3]{\prefixed{\arecv{#1}{#2}}{#3}}
\newcommand*{\close}[2]{\prefixed{\aclose{#1}}{#2}}
\newcommand*{\wait}[2]{\prefixed{\await{#1}}{#2}}
\newcommand*{\inl}[2]{\prefixed{\ainl{#1}}{#2}}
\newcommand*{\inr}[2]{\prefixed{\ainr{#1}}{#2}}
\NewDocumentCommand{\choice}{s m m m}{
	\IfBooleanTF{#1}
	{{#2}\fixspace{\triangleright}\mspace{-6mu}\left\{\mspace{-10mu}\array{rl}%
		\minl\colon&\mspace{-15mu}#3\\%
		\minr\colon&\mspace{-15mu}#4%
	\endarray\mspace{-8mu}\right\}}%
	{{#2}\fixspace{\triangleright}\mspace{-6mu}\left\{%
		\minl\colon\mspace{-4mu}#3;%
		\minr\colon\mspace{-4mu}#4\right\}}}
\NewDocumentCommand{\choicebit}{s m m m}{
	\IfBooleanTF{#1}
	{{#2}\fixspace{\triangleright}\left\{\mspace{-10mu}\array{rl}%
		0\mapsto&\mspace{-15mu}#3\\%
		1\mapsto&\mspace{-15mu}#4%
	\endarray\mspace{-8mu}\right\}}%
	{{#2}\fixspace{\triangleright}\left\{%
		0\mapsto\mspace{-4mu}#3;%
1\mapsto\mspace{-4mu}#4\right\}}}
\newcommand*{\sendtype}[3]{\prefixed{\asendtype{#1}{#2}}{#3}}
\newcommand*{\recvtype}[3]{\prefixed{\arecvtype{#1}{#2}}{#3}}
\newcommand*{\clientdisp}[2]{\prefixed{\aclientdisp{#1}}{#2}}
\newcommand*{\clientuse}[3]{\prefixed{\aclientuse{#1}{#2}}{#3}}
\newcommand*{\clientdup}[4]{\prefixed{\aclientdup{#1}{#2}{#3}}{#4}}
\newcommand*{\server}[3]{\prefixed{\bang{#1(#2)}}{#3}}

\newcommand*{\chopop}[2]{{[#1 \coloneqq #2]}}
\newcommand*{\chop}[3]{{{#3}\chopop{#1}{#2}}}
\newcommand*{\sendho}[3]{\prefixed{\asendho{#1}{#2}}{#3}}
\newcommand*{\recvho}[3]{\prefixed{\arecvho{#1}{#2}}{#3}}
\newcommand*{\invoke}[3][]{{#2}^{#1} \langle #3 \rangle}
\newcommand*{\abstr}[2]{(#1)#2}
\makeatletter
\newcommand{\pabstr}{\@ifstar{\pabstr@}{\pabstr@@}}
\newcommand*{\pabstr@}[2]{(#1)\cboxed{black!20}{%
  \let\@ots\inferTabSkip%
  \def\inferTabSkip{\hspace{1.4ex}}%
  \scriptstyle#2}}
\newcommand*{\pabstr@@}[4]{\pabstr@{#1}{\judge{#2}{#3}{#4#1}}}
\makeatother
\newcommand{\sendfree}[3]{\prefixed{\asendfree{#1}{#2}}{#3}}

\NewDocumentCommand{\hole}{o}{\IfNoValueTF{#1}{\Box}{\boxed{#1}}}
\let\ctx\mathbb


\newcommand{\co}[1]{\overline{#1}}

\newcommand*{\lsync}[2]{(#1 \parallel #2)}

\newcommand*{\lsend}[2]{{\asend{#1}{#2}}}
\newcommand*{\ltensor}[2]{{#1 \tensor #2}}
\newcommand*{\lrecv}[2]{{\arecv{#1}{#2}}}
\newcommand*{\lparr}[2]{{#1 \parr #2}}
\newcommand*{\lclose}[1]{{\aclose{#1}}}
\newcommand*{\lone}{{\one}}
\newcommand*{\lwait}[1]{{\await{#1}}}
\newcommand*{\lbot}{{\bot}}
\newcommand*{\lsendtype}[2]{{\asendtype{#1}{#2}}}
\newcommand*{\lexists}[1]{{\exists #1}}
\newcommand*{\lrecvtype}[2]{{\arecvtype{#1}{#2}}}
\newcommand*{\lforall}[1]{{\forall #1}}
\newcommand*{\linl}[1]{{\ainl{#1}}}
\newcommand*{\loplusl}[2]{{#1 \oplus_1 #2}}
\newcommand*{\lcoinl}[1]{{\acoinl{#1}}}
\newcommand*{\lwithl}[2]{{#1 \with_1 #2}}
\newcommand*{\linr}[1]{{\ainr{#1}}}
\newcommand*{\loplusr}[2]{{#1 \oplus_2 #2}}
\newcommand*{\lcoinr}[1]{{\acoinr{#1}}}
\newcommand*{\lwithr}[2]{{#1 \with_2 #2}}
\newcommand*{\lforward}[2]{{\aforward{#1}{#2}}}
\newcommand*{\laxiom}[1]{{\ref*{rule:axiom}\,{#1}}}
\newcommand*{\luse}[2]{{\aclientuse{#1}{#2}}}
\newcommand*{\lquery}[1]{{\query #1}}
\newcommand*{\lcouse}[2]{{\aserveruse{#1}{#2}}}
\newcommand*{\lbang}[1]{{\bang #1}}
\newcommand*{\ldup}[3]{{\aclientdup{#1}{#2}{#3}}}
\newcommand*{\lcontract}[1]{{\query_{\ref*{rule:contract}} #1}}
\newcommand*{\lcodup}[4][]{{\aserverdup{#2}{#3}{#4}_{#1}}}
\newcommand*{\lcocontract}[1]{{\bang_{\ref*{rule:contract}} #1}}
\newcommand*{\ldisp}[1]{{\aclientdisp{#1}}}
\newcommand*{\lweaken}[1]{{\query_{\ref*{rule:contract}} #1}}
\newcommand*{\lcodisp}[2][]{{\aserverdisp{#2}_{#1}}}
\newcommand*{\lcoweaken}[1]{{\bang_{\ref*{rule:contract}} #1}}

\newcommand*{\lsendho}[2]{{\asendho{#1}{#2}}}
\newcommand*{\lprovide}[1]{{\provide{#1}}}
\newcommand*{\lrecvho}[2]{{\arecvho{#1}{#2}}}
\newcommand*{\lassume}[1]{{\assume{#1}}}

\newcommand*{\lsubst}[3][]{\chopop{{#2}^{#1}}{#3}}
\newcommand*{\lchop}[2]{{#1\nohl{\seq\ccolon}#2}}

\def\plbl#1#2{#1}

\def\pw{\mathcal{P}}
\def\lb{\mathcal{L}}
\let\der\prf
\def\ActSet{{Act}}
\def\LblSet{{Lbl}}
\def\DerSet{{Der}}
\def\ProcSet{{Proc}}
\def\EnvSet{{Env}}
\def\proc{{proc}}
\def\env{{env}}
\newcommand{\hoenv}[2]{{\langle\thl{#1};\thl{#2}\rangle}}
\def\Set{\mathsf{Set}}

